Hyperparametric Robust and Dynamic Influence Maximization

We study the problem of robust influence maximization in dynamic diffusion networks. In line with recent works, we consider the scenario where the network can undergo insertion and removal of nodes and edges, in discrete time steps, and the influence weights are determined by the features of the corresponding nodes and a global hyperparameter. Given this, our goal is to find, at every time step, the seed set maximizing the worst-case influence spread across all possible values of the hyperparameter. We propose an approximate solution using multiplicative weight updates and a greedy algorithm, with provable quality guarantees. Our experiments validate the effectiveness and efficiency of the proposed methods.

==> checklist.tex <==
\section*{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. yes%(yes/partial/no/NA)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. yes%(yes/no)
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper. yes%(yes/no)
\end{itemize}

Does this paper make theoretical contributions? yes%(yes/no)

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. yes%(yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). yes%(yes/partial/no)
    \item Proofs of all novel claims are included. yes%(yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. yes%(yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. yes%(yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. yes%(yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. NA%(yes/no/NA)
\end{itemize}

Does this paper rely on one or more datasets? yes%(yes/no)

If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. yes%(yes/partial/no/NA)
    \item All novel datasets introduced in this paper are included in a data appendix. yes%(yes/partial/no/NA)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. yes%(yes/partial/no/NA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. yes%(yes/no/NA)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. yes%(yes/partial/no/NA)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA%(yes/partial/no/NA)
\end{itemize}

Does this paper include computational experiments? yes%(yes/no)

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. yes%(yes/partial/no)
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. yes%(yes/partial/no)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. yes%(yes/partial/no)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. yes%(yes/partial/no)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. yes%(yes/partial/no/NA)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. yes%(yes/partial/no)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. yes%(yes/partial/no)
    \item This paper states the number of algorithm runs used to compute each reported result. yes%(yes/no)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. yes%(yes/no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). no%(yes/partial/no)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. yes%(yes/partial/no/NA)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. yes%(yes/partial/no/NA)
\end{itemize}

==> full.tex <==
\section{Solution -- Fully Dynamic setting}
\label{sec:full}


In the fully dynamic setting, where any of the four changes in \S~\ref{sec:dynamic} can take place at every time step, it is hard to obtain a good approximation with a reasonable running time (\S~\ref{sec:problem}). Thus, the same holds for the fully dynamic setting where there is noise in the edge probabilities. In this section, we design a heuristic solution to Problem \ref{prob:rob_dyn_im} under the fully dynamic setting. To the best of our knowledge, this represents the first study on algorithmic solutions for the fully dynamic setting that are robust to noise in the edge probabilities. 


%As mentioned in \S~\ref{sec:contribution}, this is another of our novel contributions as we are the first to propose a solution to this problem.

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Remove-Node}}
	\begin{algorithmic}[1]
		\REQUIRE Vertex $u \in V$
		% \ENSURE 
        \STATE $V \gets V \setminus \{u\}$, $n \gets n - 1$
        \IF{$n \leq n_0 / 2$}
        \STATE $m_0 \gets m$, $n_0 \gets n$
        \STATE \textsc{Restart}
        \ELSE
        \FOR{$i = 1$ \TO $l$}
        \STATE $V_{L,est,i} \gets V_{L,est,i} \setminus \{u\}$
        \STATE $V_{L,cv,i} \gets V_{L,cv,i} \setminus \{u\}$
        \STATE $V_{R,est,i} \gets V_{R,est,i} \setminus \{u\}$
        \STATE $V_{R,cv,i} \gets V_{R,cv,i} \setminus \{u\}$
        \ENDFOR
        \ENDIF
	\end{algorithmic}
	\label{alg:remove_node}
\end{algorithm}

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Remove-Edge}}
	\begin{algorithmic}[1]
		\REQUIRE Edge $e = (u, v) \in E$
		% \ENSURE 
        \STATE $E \gets E \setminus \{e\}$, $m \gets m - 1$
        \IF{$m \leq m_0 / 2$}
        \STATE $m_0 \gets m$, $n_0 \gets n$
        \STATE \textsc{Restart}
        \ELSE
        \FOR{$i = 1$ \TO $l$}
        \FORALL{$v' \in V_{R,est,i}$}
        \IF{$(v, v') \in E_{est,i}$ \AND $(u, v') \in E_{est,i}$}
        \STATE Reduce RR sets $R_{v',est,i}$% to $R_{v',est,i}^{new}$
        % \STATE $R_{v',est,i}^{new} \gets R_{v',est,i}$
        \IF{\#edges scanned to update $\mathcal{H}_{est,i} \geq 16Rm_0$}
        \STATE \textsc{Restart}
        \ENDIF
        \ENDIF
        \ENDFOR
        \ENDFOR
        \FORALL{$(u', v') \in V \times V$}
        \STATE $I(u', v') \gets \emptyset$
        \ENDFOR
        \FOR{$i = 1$ \TO $l$}
        \FORALL{$v' \in V_{R,cv,i}$}
        \IF{$(v, v') \in E_{cv,i}$ \AND $(u, v') \in E_{cv,i}$}
        \STATE Reduce RR sets $R_{v',cv,i}$ to $R_{v',cv,i}^{new}$
        \FORALL{$u' \in R_{v',cv,i}^{new} \setminus R_{v',cv,i}$}
        \STATE $I(u', v') \gets I(u', v') \cup \{i\}$
        \ENDFOR
        \STATE $R_{v',cv,i}^{new} \gets R_{v',cv,i}$
        \ENDIF
        \ENDFOR
        \ENDFOR
        \FORALL{$(u', v') \in V \times V$}
        \FORALL{$i \in I(u', v')$}
        \STATE $E_{cv, i} \gets E_{cv, i} \setminus \{(u', v')\}$
        \ENDFOR
        \STATE \textsc{Find-Seeds}($(u', v')$)
        \ENDFOR
        \ENDIF
	\end{algorithmic}
	\label{alg:remove_edge}
\end{algorithm}

\subsection{Algorithm}

For insertions, the method remains the same as in \S~\ref{sec:half}. The techniques for handling  node and edge removal are shown in Algorithms \ref{alg:remove_node} -- \textsc{Remove-Node} and \ref{alg:remove_edge} -- \textsc{Remove-Edge} respectively. In both cases, a process restarts from scratch (Algorithm \ref{alg:restart}) whenever the number of nodes or edges is halved. A node removal only leads to its removal from all RR sets. When an edge $(u, v)$ is removed, however, the diffusion pathways can be affected, and thus more processing is needed. Specifically, we need to reduce each RR set containing both $u$ and $v$, where $u$ was reached after sampling incoming edges to $v$, by removing $u$ and all of its descendants in the RR set.\footnote{For this, we need to store the graph structure of each RR set while it is generated.} For RR sets in $\mathcal{H}_{est,i}$, if this process results in the overall number of edges in $E$ scanned while updating $\mathcal{H}_{est}$ exceeding\footnote{Removing a node and all of its descendants from an RR set requires scanning the edges in the graph structure of the RR set, which leads to the increase in the number of edges in the network scanned while updating the corresponding coverage graph.} a threshold, we restart from scratch (Algorithm \ref{alg:restart}). For RR sets in $\mathcal{H}_{cv,i}$, such an RR set reduction leads to the removal of (bipartite) edges, which requires an update of the seed set. The seed set is computed by calling the same MWU-based  method as for insertions (Algorithm \ref{alg:find_seeds}). However, the approximation algorithm called in line \ref{line:greedy} of Algorithm \ref{alg:find_seeds} is different for edge removals. When an edge $(u',v') \in E_{cv,i}$ is to be removed, for each thread, we remove $u'$ from the seed set if its marginal loss in score is above a threshold; after that, we add the node with the maximum marginal gain if it is above the threshold. This is shown in Algorithm \ref{alg:greedy_remove} -- \textsc{Greedy (Removal)}.


\subsection{Analysis}

We first provide a quality guarantee for our modified greedy algorithm, which is Algorithm \ref{alg:greedy_insert} or \ref{alg:greedy_remove} depending on whether an edge is inserted or removed (proof in Appendix \ref{sec:proof_greedy_full}). 
Consider a run of the algorithm on the addition (resp. removal) of a node to (resp. from) an RR set, with the input objective function $F$ being a linear combination (defined by weight vector $w$) of the $l$ sampled influence functions. For any seed set $S$ and $x < |S|$, let $S_{1:x}$ denote the set of the first $x$ nodes added to $S$. Also, for $x < y < |S|$, let $F_{t_y}(S_{1:x})$ denote the value of $F(S_{1:x})$ at the time the $y^{\text{th}}$ node was added to $S$. 

\begin{lemma}
\label{lem:greedy_full}
    Algorithm \ref{alg:greedy_insert} or \ref{alg:greedy_remove} (depending on insertion or removal) returns a seed set $\hat{S}$ such that $F\left(\hat{S}\right) \geq (\gamma - \epsilon_1) \cdot OPT$, i.e. guarantees a $(\gamma - \epsilon_1)$-approximation, where
    \begin{small}
    \vspace{-2mm}
    \begin{equation*}
       \gamma = \left( 1 - \frac{1}{e} \right) - \sum_{x=1}^{\left| \hat{S} \right|} \frac{F_{t_x} \left( \hat{S}_{1:x} \right) - F_{t_{x+1}} \left( \hat{S}_{1:x} \right)}{OPT} \left( 1 - \frac{1}{k} \right)^{k - x}
   \end{equation*}
    \end{small}
\end{lemma}

As in \S~\ref{sec:analysis}, to check how close the above approximation guarantee is to $1 - 1/e - \epsilon_1$, we ran simulations and computed the maximum value of the difference between the two values. We found that that value was XXX. This shows that this algorithm approximates very well in practice.

We now provide the quality guarantee and the amortized running time of our overall method with each network update for the fully dynamic setting in Theorem \ref{th:runtime}. The proof is analogous to that of Theorem \ref{th:i2theta}.

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Greedy (Removal)}}
	\begin{algorithmic}[1]
		\REQUIRE Objective function $F$, edge $(u', v')$
		% \ENSURE 
        \FOR{$i = 0$ \TO $\lceil \epsilon^{-1} \log n \rceil$}
        % \STATE $S_i \gets$ Last stored seed set for thread $i$
        \STATE $S_i \gets S_i \setminus \{u'\}$
        \STATE $u'' \gets \argmax_{v'' \notin S_i} F(S_i \cup \{v''\}) - F(S_i)$
        \REPEAT
        \STATE $S_i \gets S_i \cup \{u''\}$
        \STATE $u'' \gets \argmax_{v'' \notin S_i} F(S_i \cup \{v''\}) - F(S_i)$
        \UNTIL{$F(S_i \cup \{u''\}) - F(S_i) \geq [(1 + \epsilon_1)^i - F(S_i)] / k$ \AND $|S_i| < k$}
        \ENDFOR
        \RETURN $\arg\max_{i} F(S_i)$
	\end{algorithmic}
	\label{alg:greedy_remove}
\end{algorithm}

\vspace{-1.5mm}
\begin{theorem}
\label{th:runtime}
    Let $\gamma$ be as defined in Lemma \ref{lem:greedy_full}. Let $c_p$ denote the maximum number of phases during which the size of the graph remains within a factor of 2 of the original. Within each such phase, let $c_r$ denote the number of stages within which the number of edges scanned to update $\mathcal{H}_{est,i}$ for each $i \in [l]$ remains below the threshold after which it restarts from scratch. With probability at least $1 - \delta_1 - \delta_2$, in every time step $t$,
    \begin{small}
    \begin{equation*}
        \min_{\theta \in \Theta} \sigma_{\theta, t} (S_{tc}) \geq \left( \gamma - 3\epsilon_1 \right) \max_{S \subseteq V_t : |S| \leq k} \min_{\theta \in \Theta} \sigma_{\theta, t} (S) - 2\epsilon_2
    \end{equation*}
    \end{small}
    for $l \geq d \left( \frac{2Bdmn}{\epsilon_2} \right)^d \log \left( \frac{2Bdmn}{\epsilon_2\delta_2} \right)$ and $T \geq \frac{2 \log l}{\epsilon_2^{2}}$, with amortized running time $O \left( \frac{n^2 l^2 T c_p c_r}{k^2 \epsilon_1^3} \cdot \log n \cdot \log \left( \frac{n^{Tk}}{\delta_1} \right) \right)$.
\end{theorem}
\vspace{-1.5mm}

For the incremental setting, the size of the network can increase by a factor of at most $2$ between consecutive restarts, using which it can be shown that the values of $c_p$ and $c_r$ in Theorem \ref{th:runtime} are at most $O(\log n)$ \cite{peng2021dynamic}, leading to the running time being as in Theorem \ref{th:i2theta}. But the same does not hold for the fully dynamic setting. Also, in the incremental setting, according to Line \ref{line:cond_k} of Algorithm \ref{alg:greedy_insert}, once all threads' seed sets have $k$ nodes each, they will not be further updated (since they can only increase in size), which means we can also avoid bookkeeping computations like updating the marginal gain of every node for subsequent seed additions. However, this cannot be done for the fully dynamic setting because, in that case, even if a thread's seed set has $k$ nodes, an edge deletion will require replacement of one seed with another, which requires the marginal gains of each node to be up to date (Algorithm \ref{alg:greedy_remove}). These factors account for the running time being longer for the fully dynamic setting than for the incremental setting, as validated empirically in \S~\ref{sec:results}.

==> half.tex <==
\vspace{-1mm}
\section{Solution -- Incremental Setting}
\label{sec:half}
\vspace{-1mm}
In this section, we propose an approximate solution to Problem \ref{prob:rob_dyn_im} under the \emph{incremental} setting where, at each time step, a node or an edge can only be inserted (not removed) from the network. We discuss the overall algorithm in \S~\ref{sec:algorithm} and conduct a theoretical analysis of the solution's quality and running time in \S~\ref{sec:analysis}.% As mentioned in \S~\ref{sec:contribution}, the accuracy guarantees constitute some of our novel contributions since they are not trivial extensions of those in prior works.

\vspace{-1mm}
\subsection{Algorithm}
\label{sec:algorithm}
We first provide a brief overview of our method. Let $n_0$ and $m_0$ respectively denote the initial number of nodes and edges in our network. As mentioned in the last paragraph of \S~\ref{sec:robust}, we first sample $l$ values $\theta_1, \ldots, \theta_l$ from the hyperparameter space $\Theta$. Then, for each sampled hyperparameter, following the \eat{bulk of the IM literature} state of the art in IM, we sample a few reverse reachable (RR) sets and solve a maximum coverage problem on those sets, thereby computing the seed set for the initial network. After that, when a node or an edge is added to the network, we generally run some incremental computations, e.g. augmenting the previously generated RR sets and hence the seed sets. However, if some conditions are satisfied after the network update (e.g., the size of the network is doubled), we restart from scratch. In the next  paragraphs, we explain our method in more details.

When our method runs for the very first time, for each $i \in [l]$, it invokes Algorithm \ref{alg:restart} -- \textsc{Restart} where, from each node $v$, it generates two RR sets $R_{v,est,i}$ and $R_{v,cv,i}$ (lines \ref{line:begin_gen_rr}-\ref{line:end_gen_rr}), each with probability $p_i$ (computed in lines \ref{line:begin_p}-\ref{line:end_p})\footnote{Note that the value of $p_i$ computed in Algorithm \ref{alg:restart} can be greater than $1$. In that case, from each node $v$, we generate $\lfloor p_i \rfloor$ RR sets with probability 1 and an additional RR set with probability $p_i - \lfloor p_i \rfloor$. The value of $p_i$ is computed and RR sets are sampled accordingly in such a way that, irrespective of whether or not $p_i$ is more than 1 (there are multiple RR sets from each node), the coverage normalised by $p_i$ is an unbiased estimate of the true spread, and hence the subsequent quality guarantees hold. This is the setting in \cite{peng2021dynamic} and is similar to classic IM \cite{TXS14, TSX15} where the number of randomly chosen nodes is such that, even if there are multiple RR sets from some nodes, the estimated spread is unbiased.}. These collections of RR sets are modelled as bipartite coverage graphs $\mathcal{H}_{est,i} = (V_{L,est,i}, V_{R,est,i}, E_{est,i})$ and $\mathcal{H}_{cv,i} = (V_{L,cv,i}, V_{R,cv,i}, E_{cv,i})$, where $(u, v) \in E_{est,i}$ (resp. $E_{cv,i}$) if and only if $u \in R_{v,est,i}$ (resp. $R_{v,cv,i}$). The reason behind generating two bipartite graphs is to decouple the correlation between estimating the influence spread of a seed set and estimating the time required to sample an RR set \cite{peng2021dynamic}. $\mathcal{H}_{cv,i}$ is used for the former, while $\mathcal{H}_{est,i}$ is used for the latter. Clearly, the number of RR sets $R_{v,cv,i}$ covered by a seed set $S$ is equal to the number of nodes in $V_{R,cv,i}$ adjacent to $S$ in $\mathcal{H}_{cv,i}$. This number, normalized (divided) by $p_i$, is denoted by $f_{cv,i}(S)$ and is used to estimate the true influence spread $\sigma_{\theta_i}(S)$ of $S$ for hyperparameter $\theta_i$.

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Restart}}
	\begin{algorithmic}[1]
		% \REQUIRE 
		% \ENSURE 
        \STATE $\delta \gets n_0 \left( \delta_1/(16(2n_0)^{Tk}) \right) ^{(12n_0^2)/(ck^3)}$
        \STATE $R \gets ck\epsilon_1^{-2} \log \left( n_0 / \delta \right)$
        \FOR{$i = 1$ \TO $l$} \label{line:begin_p}
        \STATE $K_i \gets 0$
        \REPEAT
        \STATE Sample RR set with hyperparameter $\theta_i$ uniformly over $V_t$
        \STATE $K_i \gets K_i + 1$
        \UNTIL{$Rm_0$ edges are checked}
        \STATE $p_i \gets \frac{K_i}{n_0}$
        \ENDFOR \label{line:end_p}
        \FORALL{$(u, v) \in V \times V$}
        \STATE $I(u, v) \gets \emptyset$
        \ENDFOR
        \FOR{$i = 1$ \TO $l$} \label{line:begin_gen_rr}
        \FORALL{$v \in V$}
        \STATE Generate RR set $R_{v,est,i}$ with probability $p_i$
        \STATE Generate RR set $R_{v,cv,i}$ with probability $p_i$
        \FORALL{$u \in R_{v,cv,i}$}
        \STATE $I(u, v) \gets I(u, v) \cup \{i\}$
        \ENDFOR
        \ENDFOR
        \ENDFOR \label{line:end_gen_rr}
        \FORALL{$(u, v) \in V \times V$} \label{line:begin_find}
        \FORALL{$i \in I(u, v)$}
        \STATE $E_{cv, i} \gets E_{cv, i} \cup \{(u, v)\}$
        \ENDFOR
        \STATE \textsc{Find-Seeds}($(u, v)$)
        \ENDFOR \label{line:end_find}
	\end{algorithmic}
	\label{alg:restart}
% \vspace{-3mm}
\end{algorithm}
%\vspace{-5mm}
\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Find-Seeds}}
	\begin{algorithmic}[1]
		\REQUIRE $(u', v')$
		\ENSURE Seed set
        \FOR{$j = 1$ \TO $T$}
        \FOR{$i = 1$ \TO $l$}
        \STATE $w_j[i] \propto \exp \left( -\eta \sum_{\tau=1}^{j-1} f_{cv,i} (S^{(\tau)}) \right)$
        \ENDFOR
        \STATE $S^{(j)} \gets$ Greedy($\langle w_j, f_{cv} \rangle, (u', v')$) \label{line:greedy}
        \ENDFOR
        \FOR{$i = 0$ \TO $\lceil \epsilon^{-1} \log n \rceil$}
        \STATE $S_i \gets$ Seed set computed by \textsc{Greedy (Insertion)} for thread $i$ with uniform weights
        \ENDFOR
        \RETURN Uniform distribution over $\left\{ S^{(1)}, \ldots, S^{(T)} \right\}$
        % \STATE $S \gets \bigcup_{j=1}^T S^{(j)}$
	\end{algorithmic}
	\label{alg:find_seeds}
\end{algorithm}

We now discuss how to find the seed set via dynamic maximum coverage on the $\mathcal{H}_{cv,i}$s. As shown in lines \ref{line:begin_find}-\ref{line:end_find} of Algorithm \ref{alg:restart}, whenever an edge is added to the $\mathcal{H}_{cv,i}$s (i.e., a node is added to the corresponding RR sets), the seed set also needs to be updated by invoking Algorithm \ref{alg:find_seeds} -- \textsc{Find Seeds}. Along the lines of \cite{kalimeris2019robust}, Algorithm \ref{alg:find_seeds} -- \textsc{Find Seeds} runs $T$ iterations of multiplicative weight updates (MWU). Each iteration computes a candidate seed set, after running an approximation algorithm to maximize a convex combination $F$ of the sampled influence functions (line \ref{line:greedy}), with higher weights being given to those with poor performance in previous iterations\footnote{This is because our objective is to maximize the minimum influence spread.}. Similar to \cite{peng2021dynamic}, the approximation algorithm used in line \ref{line:greedy} of Algorithm \ref{alg:find_seeds}, which is shown in Algorithm \ref{alg:greedy_insert} -- \textsc{Greedy (Insertion)}, maintains a seed set for each of the $\lceil \epsilon^{-1} \log n \rceil$ threads, where thread $i$ corresponds to the estimate $(1 + \epsilon_1)^i$ of the maximum value of $F$. Algorithm \ref{alg:greedy_insert} adds to each thread's seed set any node with marginal gain above a threshold. After that, it returns the seed set maximizing $F$. In the end,  after getting the candidate seed sets using MWU, Algorithm \ref{alg:find_seeds} returns one of those sets uniformly at random, after updating each thread's seed set to be the last one computed by Algorithm \ref{alg:greedy_insert}, with $F$ having uniform weights.

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Greedy (Insertion)}}
	\begin{algorithmic}[1]
		\REQUIRE Objective function $F$, edge $(u', v')$
		\ENSURE Seed set
        \FOR{$i = 0$ \TO $\lceil \epsilon^{-1} \log n \rceil$}
        % \STATE $S_i \gets$ Last stored seed set for thread $i$
        \STATE $u'' \gets u'$
        \WHILE{$F(S_i \cup \{u''\}) - F(S_i) \geq [(1 + \epsilon_1)^i - F(S_i)] / k$ \AND $|S_i| < k$} \label{line:cond_k}
        \STATE $S_i \gets S_i \cup \{u''\}$
        \STATE $u'' \gets \argmax_{v'' \notin S_i} F(S_i \cup \{v''\}) - F(S_i)$
        \ENDWHILE
        \ENDFOR
        \RETURN $\arg\max_{i} F(S_i)$
	\end{algorithmic}
	\label{alg:greedy_insert}
\end{algorithm}

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Insert-Node}}
	\begin{algorithmic}[1]
		\REQUIRE Node $u \in V$
		% \ENSURE 
        \STATE $V \gets V \cup \{u\}$, $n \gets n + 1$
        \IF{$n \geq 2n_0$}
        \STATE $m_0 \gets m$, $n_0 \gets n$
        \STATE \textsc{Restart}
        \ELSE
        \FOR{$i = 1$ \TO $l$}
        \STATE $V_{L,est,i} \gets V_{L,est,i} \cup \{u\}$
        \STATE $V_{L,cv,i} \gets V_{L,cv,i} \cup \{u\}$
        \STATE $V_{R,est,i} \gets V_{R,est,i} \cup \{u\}$ with probability $p_i$
        \STATE $V_{R,cv,i} \gets V_{R,cv,i} \cup \{u\}$ with probability $p_i$
        \ENDFOR
        \ENDIF
	\end{algorithmic}
	\label{alg:insert_node}
\end{algorithm}

\begin{algorithm}[tb!]
    \small
	\caption{\textsc{Insert-Edge}}
	\begin{algorithmic}[1]
		\REQUIRE Edge $e = (u, v) \in E$
		% \ENSURE 
        \STATE $E \gets E \cup \{e\}$, $m \gets m + 1$
        \IF{$m \geq 2m_0$}
        \STATE $m_0 \gets m$, $n_0 \gets n$
        \STATE \textsc{Restart}
        \ELSE
        \FOR{$i = 1$ \TO $l$}
        \FORALL{$v' \in V_{R,est,i}$}
        \IF{$(v, v') \in E_{est,i}$}
        \STATE Augment RR sets $R_{v',est,i}$% to $R_{v',est,i}^{new}$
        % \STATE $R_{v',est,i}^{new} \gets R_{v',est,i}$
        \IF{\#edges scanned to update $\mathcal{H}_{est,i} \geq 16Rm_0$}
        \STATE \textsc{Restart}
        \ENDIF
        \ENDIF
        \ENDFOR
        \ENDFOR
        \FORALL{$(u', v') \in V \times V$}
        \STATE $I(u', v') \gets \emptyset$
        \ENDFOR
        \FOR{$i = 1$ \TO $l$}
        \FORALL{$v' \in V_{R,cv,i}$}
        \IF{$(v, v') \in E_{cv,i}$}
        \STATE Augment RR sets $R_{v',cv,i}$ to $R_{v',cv,i}^{new}$
        \FORALL{$u' \in R_{v',cv,i}^{new} \setminus R_{v',cv,i}$}
        \STATE $I(u', v') \gets I(u', v') \cup \{i\}$
        \ENDFOR
        \STATE $R_{v',cv,i}^{new} \gets R_{v',cv,i}$
        \ENDIF
        \ENDFOR
        \ENDFOR
        \FORALL{$(u', v') \in V \times V$}
        \FORALL{$i \in I(u', v')$}
        \STATE $E_{cv, i} \gets E_{cv, i} \cup \{(u', v')\}$
        \ENDFOR
        \STATE \textsc{Find-Seeds}($(u', v')$)
        \ENDFOR
        \ENDIF
	\end{algorithmic}
	\label{alg:insert_edge}
\end{algorithm}

After the initial run, when a node (resp. edge) is inserted to the network, Algorithm \ref{alg:insert_node} -- \textsc{Insert Node} (resp. \ref{alg:insert_edge} -- \textsc{Insert Edge}) is invoked. As shown in the pseudocode, the entire process restarts from scratch (invokes Algorithm \ref{alg:restart}) when the number of nodes or edges is doubled. Unless the restarting condition is met, the only computation required when a node is inserted is creating some RR sets containing only that node. When an edge is inserted, however, it can enhance the information diffusion in the network, thus more updates are needed. Specifically, whenever an edge $(u,v)$ with probability $p_{(u,v)}$ is added, each RR set containing $v$ but not $u$ should be augmented by adding $u$ with probability $p_{(u,v)}$. If it is added, we continue augmenting this RR set, i.e., adding new nodes to the set by sampling incoming edges of $u$ and \eat{so on} repeating the same for the new ones till no further node can be reached. For RR sets in $\mathcal{H}_{est,i}$, if this process of augmentation results in the overall number of edges in $E$ scanned while updating $\mathcal{H}_{est}$ exceeding a threshold, we restart from scratch (Algorithm \ref{alg:restart}). For RR sets in $\mathcal{H}_{cv,i}$, augmentation clearly leads to new (bipartite) edges being added, which means we need to update the seed set (Algorithm \ref{alg:find_seeds}) for each such addition.

Note that the method in \cite{peng2021dynamic} needs only two coverage graphs $\mathcal{H}_{est}$ and $\mathcal{H}_{cv}$, while ours requires $l$ such pairs of graphs to account for the noise in the edge probabilities. Also, \cite{peng2021dynamic} finds seeds by invoking the greedy algorithm for maximizing coverage only once for each update to $\mathcal{H}_{cv}$, whereas to account for the edge probability noise, we need to do the same via $T$ MWU iterations, and in each iteration, we need to maximize a convex combination of $l$ coverage functions. Fortunately, we can still provide quality guarantees for the resultant method, as shown in \S~\ref{sec:analysis}.


\subsection{Analysis}
\label{sec:analysis}

Here, we theoretically analyze the solution quality and the running time of our method. Our key result is stated in Theorem~\ref{th:i2theta}, to which we lead up by establishing some important intermediate results.

We first provide a quality guarantee for Algorithm \ref{alg:greedy_insert} (proof in Appendix \ref{sec:proof_greedy_half}). 
Consider a run of the algorithm on the addition of a node to an RR set (i.e., a call to Algorithm \ref{alg:find_seeds}), with the input objective function $F$ being a linear combination (defined by weight vector $w$) of the $l$ sampled influence functions. Let $F_{aft}^{(w)}$ (resp. $F_{bef}^{(w)}$) and $OPT_{aft}^{(w)}$ (resp. $OPT_{bef}^{(w)}$) be the objective function and its optimal value for weight vector $w$ after (resp. before) adding the node to the RR set. Also, let $uni$ denote the vector with all values $1/l$.

\begin{lemma}
\label{lem:greedy_half}
    Algorithm \ref{alg:greedy_insert} returns a seed set $\hat{S}$ such that $F_{aft}^{(w)}\left(\hat{S}\right) \geq (\gamma - \epsilon_1) \cdot OPT_{aft}^{(w)}$, i.e. guarantees a $(\gamma - \epsilon_1)$-approximation, where
    \begin{small}
    \vspace{-2mm}
    \begin{gather*}
       \gamma = \left( 1 - \frac{1}{e} \right) - \frac{OPT_{bef}^{(uni)} - x}{OPT_{aft}^{(w)}} \left( 1 - \frac{1}{k} \right) ^{k-x} \\ 
        x = \min \left\{ k, OPT_{bef}^{(uni)} - \left( \ln \frac{k}{k - 1} \right)^{-1} \right\}
   \end{gather*}
    \end{small}
\end{lemma}

To check how close the approximation guarantee of Algorithm \ref{alg:greedy_insert} is to $1 - 1/e - \epsilon_1$ (the guarantee for the state of the art algorithms on IM \cite{TXS14,TSX15}), we ran simulations on five networks (\S~\ref{sec:setup}) and computed the maximum value of the difference between the two values. We found that that value was $0$ for all datasets except the two smallest ones for which it was $4.4 \times 10^{-15}$ and $4.7 \times 10^{-14}$. This shows that Algorithm \ref{alg:greedy_insert} approximates very well in practice.

Using Lemma \ref{lem:greedy_half}, Theorem 1 of \cite{kalimeris2019robust} and Lemma 3.13 of \cite{peng2021dynamic}, we can derive the following quality guarantee for Algorithm \ref{alg:find_seeds}.

\begin{lemma}
    Let $\gamma$ be as defined in Lemma \ref{lem:greedy_half}. In every time step $t$, Algorithm \ref{alg:find_seeds} returns the uniform distribution $\mathcal{U}$ over solutions $S_t^{(1)}, \ldots, S_t^{(T)}$ s.t., for $T \geq \frac{2 \log l}{\epsilon_2^2}$, with probability at least $1 - \delta_2$,
    \begin{small}
    \begin{equation*}
        \min_{i \in [l]} \mathbb{E}_{S \sim \mathcal{U}} f_{cv, i, t} \left( S \right) \geq \left( \gamma -\epsilon_1 \right) \max_{S \subseteq V_t : \left| S \right| \leq k} \min_{i \in [l]} f_{cv, i, t} ( S) - \epsilon_2
    \end{equation*}
    \end{small}
\end{lemma}
% \begin{proof}[Proof Sketch]
%     This follows from Theorem 1 of \cite{kalimeris2019robust} and Lemma 3.13 of \cite{peng2021dynamic}.
% \end{proof}

The result of the above lemma implies the following bi-criteria approximation guarantee by returning $S_{tc} = \cup_{i=1}^T S_t^{(i)}$ instead of the uniform distribution over $\left\{ S_t^{(1)}, \ldots, S_t^{(T)} \right\}$.

\begin{corollary}
\label{cor:union}
    The seed set $S_{tc} = \cup_{i=1}^T S_t^{(i)}$ has size at most $Tk$ and, with probability at least $1 - \delta_2$, satisfies
    \begin{small}
    \begin{equation*}
        \min_{i \in [l]} f_{cv, i, t} \left( S_{tc} \right) \geq \left( \gamma -\epsilon_1 \right) \max_{S_t \subseteq V_t : \left| S_t \right| \leq k} \min_{i \in [l]} f_{cv, i, t} (S) - \epsilon_2
    \end{equation*}
    \end{small}
\end{corollary}

The above result provides a guarantee on the minimum RR set coverage $f_{cv,i,t}(\cdot)$ across all values of $i$. Using that, we now provide a guarantee on the minimum true influence spread $\sigma_{\theta_i,t}(\cdot)$ across all sampled hyperparameter values (proof in Appendix \ref{sec:proof_f2sigma}).

\begin{lemma}
\label{lem:f2sigma}
    Let $\gamma$ be as defined in Lemma \ref{lem:greedy_half}. With probability at least $1 - \delta_1 / 2 - \delta_2$,
    \begin{small}
    \begin{equation*}
        \min_{i \in [l]} \sigma_{\theta_i, t} (S_{tc}) \geq \left( \gamma - 3\epsilon_1 \right) \max_{S \subseteq V_t : |S| \leq k} \min_{i \in [l]} \sigma_{\theta_i, t} (S) - \epsilon_2
    \end{equation*}
    \end{small}
\end{lemma}

Using the above, we can provide a guarantee for the minimum influence spread across the entire hyperparameter space $\Theta$. This, along with the running time, forms the overall result of this section, the proof of which is given in Appendix \ref{sec:proof_i2theta}.

\begin{theorem}
\label{th:i2theta}
    Let $\gamma$ be as defined in Lemma \ref{lem:greedy_half}. With probability at least $1 - \delta_1 - \delta_2$, in every time step $t$,
    \begin{small}
    \begin{equation*}
        \min_{\theta \in \Theta} \sigma_{\theta, t} (S_{tc}) \geq \left( \gamma - 3\epsilon_1 \right) \max_{S \subseteq V_t : |S| \leq k} \min_{\theta \in \Theta} \sigma_{\theta, t} (S) - 2\epsilon_2
    \end{equation*}
    \end{small}
    for $l \geq d \left( \frac{2Bdmn}{\epsilon_2} \right)^d \log \left( \frac{2Bdmn}{\epsilon_2\delta_2} \right)$ and $T \geq \frac{2 \log l}{\epsilon_2^{2}}$, with amortized running time $O \left( \frac{n^2 l^2 T}{k^2 \epsilon_1^3} (\log n)^3 \log \left( \frac{n^{Tk}}{\delta_1} \right) \right)$.
\end{theorem}

\spara{Remark:} (1) Theorem \ref{th:i2theta} provides minimum values of $l$ and $T$ needed for a desired solution quality, with higher values leading to better solutions. However, in our experiments (\S~\ref{sec:sensitivity}), we find that we can obtain reasonably good results even with much smaller values of $l$ and $T$, and the solution quality converges (remains nearly the same) beyond those values. Thus, in practice, we can run our method for much smaller $l$ and $T$ (and faster), while achieving a reasonably good solution. (2) Since the value of $T$ is small in practice, as explained above, the size of $S_{tc}$ is also not much larger than $k$.

